Delayed Asynchronous Iterative Graph Algorithms

Iterative graph algorithms often compute intermediate values and update them as computation progresses. Updated output values are used as inputs for computations in current or subsequent iterations; hence the number of iterations required for values to converge can potentially reduce if the newest values are asynchronously made available to other updates computed in the same iteration. In a multi-threaded shared memory system, the immediate propagation of updated values can cause memory contention that may offset the benefit of propagating updates sooner. In some cases, the benefit of a smaller number of iterations may be diminished by each iteration taking longer. Our key idea is to combine the low memory contention that synchronous approaches have with the faster information sharing of asynchronous approaches. Our hybrid approach buffers updates from threads locally before committing them to the global store to control how often threads may cause conflicts for others while still sharing data within one iteration and hence speeding convergence. On a 112-thread CPU system, our hybrid approach attains up to 4.5% - 19.4% speedup over an asynchronous approach for Pagerank and up to 1.9% - 17% speedup over asynchronous Bellman Ford SSSP. Further, our hybrid approach attains 2.56x better performance than the synchronous approach. Finally, we provide insights as to why delaying updates is not helpful on certain graphs where connectivity is clustered on the main diagonal of the adjacency matrix.

==> design_notes.tex <==
\section{Design}

\section{notes and questions to address}
\begin{itemize}
    \item How often to flush? Should this be arch dependent? Probably we need to make a convergence argument for each algo w.r.t convergence of JC and GS.
    \item How should the local vertex data `cache' be changed for SSSP, which has sparse updates, compared to Page Rank, which has dense updates?
    \item How to size buffers and local work assigned to threads? Should these be the same?
    \item How to assign work to hyperthreads?
    \item How to assign work between sockets? Should this be informed by graph partitioning ideas, even without actually partitioning the graph?
\end{itemize}


For Page Rank, we already have an implementation that buffers updates locally to a thread for the page ranks being updated. Page Rank uses a ``pull'' kernel, so it is easy to have a small array that just stores the updated scores of the vertices assigned (Statically) to a thread.

In the case of Bellman Ford SSSP, we can do the same thing. Statically assign vertices to threads, and do a pull-style operation using a transposed adjacency matrix to pull along incoming edges.

For label-correcting SSSP and delta-Stepping SSSP, we will use push-style kernels. The number of vertices to be processed in an iteration will not be constant, and we cannot statically assign vertices to threads for the entire algorithm's runtime.

In this case, should we have a local copy of all distances per thread or per group of threads, and have each threads separately store updates to their local copy?
Then do elemwise min over sections of the arrays where updates are known to have occurred.

Another algorithm to consider here is CDLP (Community Detection by Label Propagation). Each vertex ``pulls'' labels from neighbors, counting the most frequent one, and taking that label. All vertices are active in all rounds, and the algorithm converges when every vertex already has the most frequent label from its neighbors.

What about SV? In SV we process all vertices, changing our own label. Could we buffer label updates? Is this a bad idea? {\color{red}{Go for it. I think it'll work, but it wouldn't out-perform Afforest. But that's not the point is it?}}

Could we do delayed flushing with BFS?
